Globally Resonant Homoclinic Tangencies

The attractors of a dynamical system govern its typical long-term behaviour. The presence of many attractors is significant as it means the behaviour is heavily dependent on the initial conditions. To understand how large numbers of attractors can coexist, in this thesis we study the occurrence of infinitely many stable single-round periodic solutions associated with homoclinic connections in two-dimensional maps. We show this phenomenon has a relatively high codimension requiring a homoclinic tangency and `global resonance', as has been described previously in the area-preserving setting. However, unlike in that setting, local resonant terms also play an important role. To determine how the phenomenon may manifest in bifurcation diagrams, we also study perturbations of a globally resonant homoclinic tangency. We find there exist sequences of saddle-node and period-doubling bifurcations. Interestingly, in different directions of parameter space, the bifurcation values scale differently resulting in a complicated shape for the stability region for each periodic solution. In degenerate directions, the bifurcation values scale substantially slower as illustrated in an abstract piecewise-smooth $C^{1}$ map.

==> d1compute.tex <==
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{15\unitlength}
\begin{tikzpicture}[thick,scale=0.6, every node/.style={scale=0.7}]
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (49.750000\du,28.100000\du)--(49.900000\du,28.200000\du);
}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (49.750000\du,28.100000\du)--(49.900000\du,28.200000\du);
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{49.900000\du}{28.200000\du}}
\pgfpathcurveto{\pgfpoint{49.830662\du}{28.304006\du}}{\pgfpoint{49.657319\du}{28.338675\du}}{\pgfpoint{49.553312\du}{28.269338\du}}
\pgfpathcurveto{\pgfpoint{49.449306\du}{28.200000\du}}{\pgfpoint{49.414637\du}{28.026656\du}}{\pgfpoint{49.483975\du}{27.922650\du}}
\pgfpathcurveto{\pgfpoint{49.553312\du}{27.818644\du}}{\pgfpoint{49.726656\du}{27.783975\du}}{\pgfpoint{49.830662\du}{27.853312\du}}
\pgfpathcurveto{\pgfpoint{49.934669\du}{27.922650\du}}{\pgfpoint{49.969338\du}{28.095994\du}}{\pgfpoint{49.900000\du}{28.200000\du}}
\pgfusepath{fill}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{49.900000\du}{28.200000\du}}
\pgfpathcurveto{\pgfpoint{49.830662\du}{28.304006\du}}{\pgfpoint{49.657319\du}{28.338675\du}}{\pgfpoint{49.553312\du}{28.269338\du}}
\pgfpathcurveto{\pgfpoint{49.449306\du}{28.200000\du}}{\pgfpoint{49.414637\du}{28.026656\du}}{\pgfpoint{49.483975\du}{27.922650\du}}
\pgfpathcurveto{\pgfpoint{49.553312\du}{27.818644\du}}{\pgfpoint{49.726656\du}{27.783975\du}}{\pgfpoint{49.830662\du}{27.853312\du}}
\pgfpathcurveto{\pgfpoint{49.934669\du}{27.922650\du}}{\pgfpoint{49.969338\du}{28.095994\du}}{\pgfpoint{49.900000\du}{28.200000\du}}
\pgfusepath{stroke}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.498039, 0.498039, 0.498039}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.498039, 0.498039, 0.498039}
\pgfsetstrokecolor{dialinecolor}
\draw (49.950000\du,27.450000\du)--(51.200000\du,24.200000\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (51.400000\du,23.550000\du)--(51.500000\du,23.850000\du);
}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (51.400000\du,23.550000\du)--(51.386607\du,23.509822\du);
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
\fill (51.500000\du,23.850000\du)--(51.183772\du,23.691886\du)--(51.341886\du,23.375658\du)--(51.658114\du,23.533772\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (51.500000\du,23.850000\du)--(51.183772\du,23.691886\du)--(51.341886\du,23.375658\du)--(51.658114\du,23.533772\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (41.750000\du,28.050000\du)--(42.050000\du,28.250000\du);
}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (41.750000\du,28.050000\du)--(42.050000\du,28.250000\du);
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{42.050000\du}{28.250000\du}}
\pgfpathcurveto{\pgfpoint{41.980662\du}{28.354006\du}}{\pgfpoint{41.807319\du}{28.388675\du}}{\pgfpoint{41.703312\du}{28.319338\du}}
\pgfpathcurveto{\pgfpoint{41.599306\du}{28.250000\du}}{\pgfpoint{41.564637\du}{28.076656\du}}{\pgfpoint{41.633975\du}{27.972650\du}}
\pgfpathcurveto{\pgfpoint{41.703312\du}{27.868644\du}}{\pgfpoint{41.876656\du}{27.833975\du}}{\pgfpoint{41.980662\du}{27.903312\du}}
\pgfpathcurveto{\pgfpoint{42.084669\du}{27.972650\du}}{\pgfpoint{42.119338\du}{28.145994\du}}{\pgfpoint{42.050000\du}{28.250000\du}}
\pgfusepath{fill}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{42.050000\du}{28.250000\du}}
\pgfpathcurveto{\pgfpoint{41.980662\du}{28.354006\du}}{\pgfpoint{41.807319\du}{28.388675\du}}{\pgfpoint{41.703312\du}{28.319338\du}}
\pgfpathcurveto{\pgfpoint{41.599306\du}{28.250000\du}}{\pgfpoint{41.564637\du}{28.076656\du}}{\pgfpoint{41.633975\du}{27.972650\du}}
\pgfpathcurveto{\pgfpoint{41.703312\du}{27.868644\du}}{\pgfpoint{41.876656\du}{27.833975\du}}{\pgfpoint{41.980662\du}{27.903312\du}}
\pgfpathcurveto{\pgfpoint{42.084669\du}{27.972650\du}}{\pgfpoint{42.119338\du}{28.145994\du}}{\pgfpoint{42.050000\du}{28.250000\du}}
\pgfusepath{stroke}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.498039, 0.498039, 0.498039}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.498039, 0.498039, 0.498039}
\pgfsetstrokecolor{dialinecolor}
\draw (42.050000\du,27.250000\du)--(43.233693\du,24.201825\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (43.500000\du,23.700000\du)--(43.150000\du,23.600000\du);
}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (43.500000\du,23.700000\du)--(43.494782\du,23.698509\du);
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
\fill (43.150000\du,23.600000\du)--(43.459061\du,23.428299\du)--(43.630762\du,23.737361\du)--(43.321701\du,23.909061\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (43.150000\du,23.600000\du)--(43.459061\du,23.428299\du)--(43.630762\du,23.737361\du)--(43.321701\du,23.909061\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{48.850000\du}{26.450000\du}}
\pgfpathcurveto{\pgfpoint{47.350000\du}{25.100000\du}}{\pgfpoint{46.350000\du}{24.650000\du}}{\pgfpoint{43.850000\du}{26.250000\du}}
\pgfusepath{stroke}
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (33.800000\du,27.950000\du)--(34.050000\du,28.050000\du);
}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (33.800000\du,27.950000\du)--(34.050000\du,28.050000\du);
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{34.050000\du}{28.050000\du}}
\pgfpathcurveto{\pgfpoint{34.003576\du}{28.166060\du}}{\pgfpoint{33.841093\du}{28.235695\du}}{\pgfpoint{33.725033\du}{28.189272\du}}
\pgfpathcurveto{\pgfpoint{33.608974\du}{28.142848\du}}{\pgfpoint{33.539338\du}{27.980364\du}}{\pgfpoint{33.585762\du}{27.864305\du}}
\pgfpathcurveto{\pgfpoint{33.632185\du}{27.748245\du}}{\pgfpoint{33.794669\du}{27.678609\du}}{\pgfpoint{33.910728\du}{27.725033\du}}
\pgfpathcurveto{\pgfpoint{34.026788\du}{27.771457\du}}{\pgfpoint{34.096424\du}{27.933940\du}}{\pgfpoint{34.050000\du}{28.050000\du}}
\pgfusepath{fill}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{34.050000\du}{28.050000\du}}
\pgfpathcurveto{\pgfpoint{34.003576\du}{28.166060\du}}{\pgfpoint{33.841093\du}{28.235695\du}}{\pgfpoint{33.725033\du}{28.189272\du}}
\pgfpathcurveto{\pgfpoint{33.608974\du}{28.142848\du}}{\pgfpoint{33.539338\du}{27.980364\du}}{\pgfpoint{33.585762\du}{27.864305\du}}
\pgfpathcurveto{\pgfpoint{33.632185\du}{27.748245\du}}{\pgfpoint{33.794669\du}{27.678609\du}}{\pgfpoint{33.910728\du}{27.725033\du}}
\pgfpathcurveto{\pgfpoint{34.026788\du}{27.771457\du}}{\pgfpoint{34.096424\du}{27.933940\du}}{\pgfpoint{34.050000\du}{28.050000\du}}
\pgfusepath{stroke}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.498039, 0.498039, 0.498039}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.498039, 0.498039, 0.498039}
\pgfsetstrokecolor{dialinecolor}
\draw (34.050000\du,27.350000\du)--(35.000000\du,24.250000\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (35.300000\du,23.650000\du)--(35.300000\du,23.550000\du);
}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (35.300000\du,23.650000\du)--(35.300000\du,23.908579\du);
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
\fill (35.300000\du,23.550000\du)--(35.550000\du,23.800000\du)--(35.300000\du,24.050000\du)--(35.050000\du,23.800000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (35.300000\du,23.550000\du)--(35.550000\du,23.800000\du)--(35.300000\du,24.050000\du)--(35.050000\du,23.800000\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{40.700000\du}{26.300000\du}}
\pgfpathcurveto{\pgfpoint{39.500000\du}{24.500000\du}}{\pgfpoint{37.150000\du}{25.050000\du}}{\pgfpoint{35.800000\du}{26.250000\du}}
\pgfusepath{stroke}
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetmiterjoin
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{61.100000\du}{19.650000\du}}
\pgfpathcurveto{\pgfpoint{64.600000\du}{13.850000\du}}{\pgfpoint{24.850000\du}{4.150000\du}}{\pgfpoint{33.600000\du}{27.200000\du}}
\pgfusepath{stroke}
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (44.077292\du,12.601890\du)--(44.709498\du,12.601890\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (63.950000\du,20.550000\du)--(64.150000\du,20.500000\du);
}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (63.950000\du,20.550000\du)--(64.150000\du,20.500000\du);
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{64.150000\du}{20.500000\du}}
\pgfpathcurveto{\pgfpoint{64.180317\du}{20.621268\du}}{\pgfpoint{64.089366\du}{20.772853\du}}{\pgfpoint{63.968098\du}{20.803170\du}}
\pgfpathcurveto{\pgfpoint{63.846830\du}{20.833486\du}}{\pgfpoint{63.695246\du}{20.742536\du}}{\pgfpoint{63.664929\du}{20.621268\du}}
\pgfpathcurveto{\pgfpoint{63.634612\du}{20.500000\du}}{\pgfpoint{63.725563\du}{20.348415\du}}{\pgfpoint{63.846830\du}{20.318098\du}}
\pgfpathcurveto{\pgfpoint{63.968098\du}{20.287781\du}}{\pgfpoint{64.119683\du}{20.378732\du}}{\pgfpoint{64.150000\du}{20.500000\du}}
\pgfusepath{fill}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{64.150000\du}{20.500000\du}}
\pgfpathcurveto{\pgfpoint{64.180317\du}{20.621268\du}}{\pgfpoint{64.089366\du}{20.772853\du}}{\pgfpoint{63.968098\du}{20.803170\du}}
\pgfpathcurveto{\pgfpoint{63.846830\du}{20.833486\du}}{\pgfpoint{63.695246\du}{20.742536\du}}{\pgfpoint{63.664929\du}{20.621268\du}}
\pgfpathcurveto{\pgfpoint{63.634612\du}{20.500000\du}}{\pgfpoint{63.725563\du}{20.348415\du}}{\pgfpoint{63.846830\du}{20.318098\du}}
\pgfpathcurveto{\pgfpoint{63.968098\du}{20.287781\du}}{\pgfpoint{64.119683\du}{20.378732\du}}{\pgfpoint{64.150000\du}{20.500000\du}}
\pgfusepath{stroke}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.498039, 0.498039, 0.498039}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.498039, 0.498039, 0.498039}
\pgfsetstrokecolor{dialinecolor}
\draw (63.250000\du,20.850000\du)--(60.387929\du,22.061261\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (59.800000\du,22.250000\du)--(59.950000\du,22.400000\du);
}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (59.800000\du,22.250000\du)--(59.696447\du,22.146447\du);
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
\fill (59.950000\du,22.400000\du)--(59.596447\du,22.400000\du)--(59.596447\du,22.046447\du)--(59.950000\du,22.046447\du)--cycle;
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\pgfsetbuttcap
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (59.950000\du,22.400000\du)--(59.596447\du,22.400000\du)--(59.596447\du,22.046447\du)--(59.950000\du,22.046447\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (47.700000\du,29.350000\du){$U_{2}=(u_{2},v_{2})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (51.177030\du,22.606760\du){$U_{2} + \delta v_{s}$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (41.400000\du,29.200000\du){$f(U_{2})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (46.591890\du,26.054069\du){$f$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (42.850000\du,22.550000\du){$f(U_{2}+\delta v_{s})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (38.467570\du,25.952719\du){$f$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (33.350000\du,28.900000\du){$f^{2}(U_{2})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (34.650000\du,22.700000\du){$f^{2}(U_{2}+\delta v_{s})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (42.050000\du,11.650000\du){applying $f$ for $(n-2)$ times};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (64.712160\du,20.494600\du){$U_{1} = f^{n}(U_{2})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (59.627020\du,23.398650\du){$W = U_{1} + \delta v_{\text{diff}}$};
\end{tikzpicture}
    
